MultiCite: Modeling realistic citations requires moving beyond the single-sentence single-label setting

Citation context analysis (CCA) is an important task in natural language processing that studies how and why scholars discuss each others' work. Despite decades of study, traditional frameworks for CCA have largely relied on overly-simplistic assumptions of how authors cite, which ignore several important phenomena. For instance, scholarly papers often contain rich discussions of cited work that span multiple sentences and express multiple intents concurrently. Yet, CCA is typically approached as a single-sentence, single-label classification task, and thus existing datasets fail to capture this interesting discourse. In our work, we address this research gap by proposing a novel framework for CCA as a document-level context extraction and labeling task. We release MultiCite, a new dataset of 12,653 citation contexts from over 1,200 computational linguistics papers. Not only is it the largest collection of expert-annotated citation contexts to-date, MultiCite contains multi-sentence, multi-label citation contexts within full paper texts. Finally, we demonstrate how our dataset, while still usable for training classic CCA models, also supports the development of new types of models for CCA beyond fixed-width text classification. We release our code and dataset at https://github.com/allenai/multicite.

==> imbalanced-metrics.tex <==




\citet{li2014addressing} use balanced accuracy: \[
\frac{1}{k} \sum_{i=1}^n\frac{c_i}{n_i}
\]
where $k$ is the number of relations to predict, $c_i$ is the number of instances of relation $i$ that are correctly predicted, $n_i$ is the total number of instances of relation $i$.
They  argue Balanced accuracy (or averaged accuracy) has a more intuitive interpretation than F-measure.  It is not dominated by the majority class as much as standard accuracy is. For example for two classes,in a dataset where one class makes up 90\% of the data, predicting the majority class has accuracy of90\% but balanced accuracy of 45\%.


\citet{li2012active} use the g-mean \cite{kubat1997addressing} which is $\sqrt{\text{TP} \times \text{TN}}$ where TP and TN are the true positive and true negative rates. The g-mean statistic is argued to be better than F1 if all the classes are equally important and classes are heavily imbalanced.
The g-mean is implemented in the \texttt{imblearn} package.\footnote{ \url{http://glemaitre.github.io/imbalanced-learn/generated/imblearn.metrics.geometric_mean_score.html}}

\citet{dligach2011good} look at the Recall curve relative to training set sizes to visually compare but then measures accuracy for reports. They also show separate Precision and Recall results for only the rare classes (here, rare senses in a WSD  problem).

\citet{omuya2013improving} look at tagging rare dialog acts and use standard Precision, Recall, and F1.

\cite{manousogiannis2020normalization} identify drug reactions from social media and report Accuracy in a 500+ dimensional multiclass setting (I think; cf. Table 1 in their paper). They also report accuracy on the subset of the data with rare classes.

\cite{mayfield2013recognizing} are identify rare social media phenomena and report both Accuracy and $\kappa$. $\kappa$ is an interesting idea since it corrects for chance.

\cite{crammer2009multi} test on several datasets, some with tens of classes and use Accuracy.

\citet{yang2020mscnn} do multilabel classification with rare classes and report Micro F1 (which is Accuracy), Macro-averaged F1, and two ranking-based metrics NDG@k and G@k.
